oBERTa: Improving Sparse Transfer Learning via improved initialization, distillation, and pruning regimes

In this paper, we introduce the range of oBERTa language models, an easy-to-use set of language models which allows Natural Language Processing (NLP) practitioners to obtain between 3.8 and 24.3 times faster models without expertise in model compression. Specifically, oBERTa extends existing work on pruning, knowledge distillation, and quantization and leverages frozen embeddings improves distillation and model initialization to deliver higher accuracy on a broad range of transfer tasks. In generating oBERTa, we explore how the highly optimized RoBERTa differs from the BERT for pruning during pre-training and finetuning. We find it less amenable to compression during fine-tuning. We explore the use of oBERTa on seven representative NLP tasks and find that the improved compression techniques allow a pruned oBERTa model to match the performance of BERTbase and exceed the performance of Prune OFA Large on the SQUAD V1.1 Question Answering dataset, despite being 8x and 2x, respectively faster in inference. We release our code, training regimes, and associated model for broad usage to encourage usage and experimentation

==> scratchpad.tex <==

Next, we go ahead and benchmark the oBERTa model performance against existing sparse-transfer models such as oBERT and PruneOFA using the models that have been published \footnote{Since the PruneBERT model is not available in the zoo, we extrapolate numbers using the performance of our oBERTa\textsubscript{base} pruned 90\% as both models feature 12 transformer encoders and 90\% sparsity.} in Neural Magic's Sparse-Zoo \footnote{https://sparsezoo.neuralmagic.com/}. We run these models using four cores and a batch size of 1 and compare their speedup (or slowdown) relative to their performance on the SQUAD v1.1 question-answering benchmark. Results can be found in table \ref{tab:inference-competitive-short} and full results in \ref{tab:inference-competitive-full}. Looking at the improvements in accuracy and inference throughput, we find the oBERTa models are 1.3 to 4 times better than models with approximately the same accuracy.  \\
\begin{table}[!ht]
    \centering
    \scalebox{0.5}{
    \begin{tabular}{|l|l|*2l|*2l|}
    \toprule
        \multicolumn{2}{l}{} &  \multicolumn{2}{l}{Vs.\ \alex{\st{BERT\textsubscript{base}} BERT\textsubscript{base}}} & \multicolumn{2}{l}{Vs.\ \alex{\st{BERT-Large} BERT\textsubscript{LARGE}}} \\ \hline
        Model & F1 & Recovery & Speedup & Recovery & Speedup \\ \hline
        oBERTa\textsubscript{base} 90\% & 91.00 & 102.77\% & 3.57 & 100.44\% & 20.21 \\ \hline
        obert\textsubscript{LARGE 95\% Quantized & 90.21 & 101.87\% & 3.41 & 99.57\% & 19.31 \\ \hline
        \midrule
        prunedOFA\textsubscript{LARGE} 90\% Quantized & 89.96 & 101.59\% & 2.38 & 99.29\% & 13.47 \\ \hline
        oBERTa\textsubscript{base} 90\% Quantized & 89.46 & 101.03\% & 7.62 & 98.74\% & 43.07 \\ \hline
        \midrule
        oBERTa\textsubscript{MEDIUM} 90\%   & 89.26 & 98.99\% & 7.78 & 96.75\% & 43.99 \\ \hline
        obert\textsubscript{base} 90\% Quantized & 88.00 & 99.38\% & 6.96 & 97.13\% & 39.37 \\ \hline
        \midrule
        oBERTa\textsubscript{SMALL} 90\% & 84.66 & 90.97\% & 13.95 & 88.91\% & 78.91 \\ \hline
        pruneBERT & 84.90 & 95.88\% & 3.57  & 93.71\% & 73.82 \\ \hline
        
        \bottomrule
    \end{tabular}}
    \caption{Speedups of the oBERTa-family compared to existing published sparse models compared to the performance of BERT\textsubscript{base} and BERT-large. Speedup measures the reduction in latency of MS/batch. oBERTA\textsubscript{base} 90\% exceeds the accuracy of oBERT 95\% quantized despite being faster, oBERTa\textsubscript{base} 90\% quantized performs at the level of pruneOFA-large 90\% Quantized despite being 3x faster, oBERTa\textsubscript{MEDIUM} 90\% can outperform oBERT\textsubscript{base } 90\% Quantized despite being 30\% faster, and oBERTa\textsubscript{SMALL} 90\% performs on par with pruneBERT despite being nearly four times faster. }
    \label{tab:inference-competitive-short}
\end{table}
Looking at the competitive results, we find that the oBERTa-* models can deliver significant gains in performance (F1) relative to speedups. The oBERTa\textsubscript{base}Pruned 90\% Quantized model achieves an undertaking that nearly matches pruneOFA-large 90\% Quantized while delivering nearly 13x faster inference. Similarly, the oBERTA\textsubscript{SMALL} 90\%  model provides similar accuracy to PruneBERT despite being over four times faster.
